Schema Matching with Large Language Models: an Experimental Study

Large Language Models (LLMs) have shown useful applications in a variety of tasks, including data wrangling. In this paper, we investigate the use of an off-the-shelf LLM for schema matching. Our objective is to identify semantic correspondences between elements of two relational schemas using only names and descriptions. Using a newly created benchmark from the health domain, we propose different so-called task scopes. These are methods for prompting the LLM to do schema matching, which vary in the amount of context information contained in the prompt. Using these task scopes we compare LLM-based schema matching against a string similarity baseline, investigating matching quality, verification effort, decisiveness, and complementarity of the approaches. We find that matching quality suffers from a lack of context information, but also from providing too much context information. In general, using newer LLM versions increases decisiveness. We identify task scopes that have acceptable verification effort and succeed in identifying a significant number of true semantic matches. Our study shows that LLMs have potential in bootstrapping the schema matching process and are able to assist data engineers in speeding up this task solely based on schema element names and descriptions without the need for data instances.

==> sections/experimental_setup.tex <==
In this section, we will first define a benchmark that allows us to assess the performance of the foundation model on the schema matching task. Second, we will elaborate on our different approaches to prompt the foundation model. Third, we will provide an overview of the our experimental setup.

\subsection{Benchmark}%
\label{sec:benchmark}

In order to create a benchmark for a schema matching task based on a real-world example from the health domain, we reverse engineer a matching based on an implementation of an extract, transform and load (ETL) process. We inspect an ETL process that uses two well-known schemas in the medical informatics community, namely the MIMIC-IV dataset\footnote{\url{https://mimic.mit.edu/docs/iv/}} and the OHDSI OMOP Common Data Model\footnote{\url{https://ohdsi.github.io/CommonDataModel/index.html}}. The OHDSI community maintains an ETL process to transform data from MIMIC-IV to OMOP\footnote{\url{https://github.com/OHDSI/MIMIC/tree/master}}, which we use as a basis to manually identify all semantic 1:1 matches between the two schemas. We extracted a total of $48$ semantic matches between $7$ relations from MIMIV-IV and $6$ relations from OMOP. Based on this set of matches, we identified $9$ relation pairs that contain at least one semantic match. We consider each of these relation pairs a \emph{dataset} in our benchmark. Our $9$ datasets create a search space of $1839$ attribute pairs that contain $48$ true semantic matches, a problem with highly imbalanced classes.

The benchmark is completed by a name and a natural language description per table and attribute contained in the benchmark we extracted from the respective documentations. We provide both the name and descriptions as well as the reverse engineered true semantic matches in the supplementary material. \todo{make available via zenodo}

\begin{table}
	\small
	\centering
	\caption{Datasets contained in the benchmark. Each dataset has a source and a target table, both with the number of attributes and the number of attribute pairs. The last column shows the number of true semantic matches.}
	\label{tab:datasets}
	\begin{tabular}[h]{l l c l c c c}
		\hline
		\#   	 		& source 		& |source| & target 			& |target| & |pairs| & |matches| \\
		\hline
		\texttt{AdCO}	& Admissions	& 16	& Condition\_Occurrence	& 16	& 256	& 2 \\
		\texttt{AdVD}	& Admissions	& 16	& Visit\_Detail			& 19	& 304	& 5 \\
		\texttt{AdVO}	& Admissions	& 16	& Visit\_Occurrence		& 17	& 272	& 8 \\
		\texttt{DiCO}	& Diagnoses\_ICD& 5		& Condition\_Occurrence	& 16	& 80	& 2 \\
		\texttt{LaMe}	& Labevents		& 10	& Measurement			& 20	& 200	& 10 \\
		\texttt{PaPe}	& Patients		& 6		& Person				& 18	& 108	& 5 \\
		\texttt{PrDE}	& Prescriptions	& 17	& Drug\_Exposure		& 23	& 391	& 6 \\
		\texttt{SeVD}	& Services		& 5		& Visit\_Detail			& 19	& 95	& 5 \\
		\texttt{TrVD}	& Transfers		& 7		& Visit\_Detail			& 19	& 133	& 6 \\
		\hline
	\end{tabular}
\end{table}

\subsection{Prompt engineering}%
\label{sec:prompting_engineering}

Foundation models are trained to answer questions in natural language. As such, we need to interface with the model via prompts based on information about tables and attributes from the benchmark. Researchers devoted significant effort to engineer prompts that convey tasks efficiently, down to single characters that increase or decrease the quality of its answers \cite{narayanCanFoundationModels2022}. Our focus lies on evaluating prompt designs. Therefore, we scanned for common practices that have shown to increase the quality of answers from the field of prompt engineering. We employ the \emph{Persona Pattern} to let the foundation model act as a schema matcher \cite{whitePromptPatternCatalog2023}. With \emph{Meta Language Creation}, we introduce our definition (see Theorem~\ref{thm:schema_matching}) to the model \cite{whitePromptPatternCatalog2023}. We reuse the prompt engineering work from \cite{narayanCanFoundationModels2022} to serialize relational schema information. The authors of \todo{work it out step by step citation} contributed the ``step-by-step'' phrase that has shown to increase performance by letting foundation models reason for a longer time. Finally, we employ the \emph{Output Automater} pattern to instruct the model to output structured data \cite{whitePromptPatternCatalog2023}.

Analogous to the input, foundation models are trained to output natural language text. We can instruct a model to create structured output in order to allow us to process the results automatically. A simple, yet effective, approach is to search for the word ``yes'' within the output of the model \cite{narayanCanFoundationModels2022,peetersUsingChatGPTEntity2023}. While this approach is feasible when asking for a single pair of attributes, asking for multiple pairs is not. Therefore, we have chosen to demand JSON-structured output summary from the model, which allows us to ask for more complex answers while retaining the natural language reasoning given by the model. During our experiments, we found that using a three-step scale for the output works best. We aks the model to use \texttt{yes} for a match, \texttt{no} for a non-match, and \texttt{unknown} if there is not enough information to decide. We also experimented with numerical scores, where we had difficulty to interpret them, and five-step scales, which were much more prone to hallucinations.

\subsection{Prompt designs}%
\label{sec:prompt_designs}

We design our prompt as follows. First, we introduce the problem to the model, using the \emph{Persona Pattern} and \emph{Meta Language Creation}. Then, we input the serialized schema information. Finally, we use the \todo{magicPhraseName} phrase and the \emph{Output Automater} pattern to finalize our task to the model. We define four different prompt designs, based on the amount of schema information that we use within a single prompt.
\begin{description}
	\item[1-to-1] Each prompt contains exactly one attribute pair.
	\item[1-to-N] Each prompt contains a single attribute from the source schema and all
		$N$ attributes of a target relation from the target schema.
	\item[N-to-1] Each prompt contains all $N$ attributes of a source relation from the
		source schema and a single attribute from the target schema.
	\item[N-to-M] Each prompts contains all $N$ attributes from a source and $M$
		attributes from a target relation from their respective schemas.
\end{description}
It is worth noting that the prompt design choice has implications on the complexity to  parse structured votes from an answer given from a foundation model. While we expect a  single vote (e.g. \texttt{yes} or \texttt{no}) in the \emph{1-to-1} case, an answer to  the \emph{N-to-M} prompt design potentially contains $N\times M$ votes, one for each attribute pair.

\subsection{Baseline}%
\label{sec:baseline}

We compare the results of our foundation model approach against a baseline calculated by the Jaro string similarity of the attribute names. Jaro is a well-known and established metric that performed best on our benchmark judged by the F1-score. To determine a threshold, we calculate the Jaro similarity of all attribute pairs per dataset and pick the threshold that achieves the best F1-score. While this approach results in a relatively unrealistic baseline in the sense that a data engineer cannot know which threshold to use in practice, it allows us to compare the foundation model against a deterministic approach.

\subsection{Methodology}%
\label{sec:methodology}

Each experiment consists of a single prompt design, which we send to the model three times. From these three answers, we extract three \emph{votes} that we summarize by major voting to minimize the effect of hallucinations. If an attribute pair prompted is missing from the result or if we have a split decision, we consider this attribute pair \texttt{unknown}. Each experiment is repeated five times. The results of the experiments are compared against our benchmark by the means of \emph{F1}-score, the harmonic mean between \emph{precision} and \emph{recall} of the true semantic matches, and an \emph{completeness}-score, indicating the amount of non-\texttt{unknown} votes. By default, we use OpenAIs \texttt{gpt-3.5-turbo-0125} model with all settings set to default.

\todo{is the following needed somewhere? could be handy to formalize the scores}

Our benchmark $\mathcal{B}$ consists of $9$ datasets $R$. Each dataset consists of all attribute pairs $(a, b)$ of two relations $A$ and $B$ such that $a \in A$ and $b \in B$. We can split each $R$ into two distinct sets, $R^+$ and $R^-$, where $R^+$ contains all $(a, b)$ where $a \cong b$ with $\cong$ denoting a semantic match between $a$ and $b$ \cite{DBLP:journals/vldb/RahmB01}. Consequently, $R^-$ contains all $(a, b)$ where $a \not\cong b$. Given a set of predictions $\mathcal{P}$ for dataset $R$ from a foundation model, which contains triples $(a, b, v)$, where $a \in A$, $b \in B$, and $v \in \{\texttt{yes}, \texttt{unknown}, \texttt{no}\}$. Analogous, we can define $\mathcal{P}^+$ as the set of attribute pairs where $v$ is \texttt{yes} and $\mathcal{P}^-$ is the set of attribute pairs where $v$ is \texttt{no}. We can define the following scores. The precision is $P(\mathcal{P}) := \frac{|\mathcal{P}^+ \cap R_i^+|}{|\mathcal{P}^+|}$, the recall is $R(\mathcal{P}) := \frac{|\mathcal{P}^+ \cap R_i^+|}{|R^+|}$. The harmonic mean of precision and recall, the F1-score, is thus 
$$
	F1(\mathcal{P}) := 
	\begin{cases}
		\frac{2 \times P(\mathcal{P}) \times R(\mathcal{P})}{P(\mathcal{P}) + R(\mathcal{P})} & \text{if } P(\mathcal{P}) + R(\mathcal{P}) > 0\\
		0.0 & \text{otherwise}
	\end{cases}
$$
Finally, we define the completeness-score as $C(\mathcal{P}) := \frac{|\mathcal{P}^+ \cup \mathcal{P}^-|}{|R|}$.


==> tables/complementarity.tex <==
AdCO & 1 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!0.0} 0 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!0.0} 0 \\
AdVD & 3 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!33.333333333333336} 1 & \cellcolor{heatmapgreen!0.0} 0 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!33.333333333333336} 1 & \cellcolor{heatmapgreen!0.0} 0 \\
AdVO & 6 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!33.333333333333336} 2 & \cellcolor{heatmapgreen!83.33333333333333} 5 & \cellcolor{heatmapgreen!16.666666666666668} 1 &  & \cellcolor{heatmapgreen!50.0} 3 & \cellcolor{heatmapgreen!83.33333333333333} 5 & \cellcolor{heatmapgreen!33.333333333333336} 2 \\
DiCO & 1 &  & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!100.0} 1 &  & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!100.0} 1 & \cellcolor{heatmapgreen!100.0} 1 \\
LaMe & 8 &  & \cellcolor{heatmapgreen!37.5} 3 & \cellcolor{heatmapgreen!50.0} 4 & \cellcolor{heatmapgreen!87.5} 7 & \cellcolor{heatmapgreen!37.5} 3 &  & \cellcolor{heatmapgreen!75.0} 6 & \cellcolor{heatmapgreen!100.0} 8 & \cellcolor{heatmapgreen!50.0} 4 \\
PaPe & 2 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!50.0} 1 & \cellcolor{heatmapgreen!50.0} 1 & \cellcolor{heatmapgreen!0.0} 0 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!50.0} 1 & \cellcolor{heatmapgreen!0.0} 0 \\
PrDE & 3 &  & \cellcolor{heatmapgreen!33.333333333333336} 1 & \cellcolor{heatmapgreen!100.0} 3 & \cellcolor{heatmapgreen!33.333333333333336} 1 & \cellcolor{heatmapgreen!0.0} 0 &  & \cellcolor{heatmapgreen!66.66666666666667} 2 & \cellcolor{heatmapgreen!66.66666666666667} 2 & \cellcolor{heatmapgreen!33.333333333333336} 1 \\
SeVD & 4 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!25.0} 1 & \cellcolor{heatmapgreen!50.0} 2 & \cellcolor{heatmapgreen!0.0} 0 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!25.0} 1 & \cellcolor{heatmapgreen!0.0} 0 \\
TrVD & 2 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 &  & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 & \cellcolor{heatmapgreen!0.0} 0 \\
\midrule
sum & 30 &  & \cellcolor{heatmapgreen!16.666666666666668} 5 & \cellcolor{heatmapgreen!40.0} 12 & \cellcolor{heatmapgreen!63.333333333333336} 19 & \cellcolor{heatmapgreen!16.666666666666668} 5 &  & \cellcolor{heatmapgreen!40.0} 12 & \cellcolor{heatmapgreen!66.66666666666667} 20 & \cellcolor{heatmapgreen!26.666666666666668} 8 \\


==> tables/consistency_std.tex <==
AdCO & & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) & \cellcolor{heatmapgreen!85} 0.052 \scriptsize (0.03, 0.27) & \cellcolor{heatmapgreen!90} 0.035 \scriptsize (0.02, 0.00) & \cellcolor{heatmapgreen!44} 0.203 \scriptsize (0.14, 0.42) &  & \cellcolor{heatmapgreen!91} 0.030 \scriptsize (0.04, 0.00) & \cellcolor{heatmapgreen!77} 0.081 \scriptsize (0.05, 0.22) & \cellcolor{heatmapgreen!67} 0.119 \scriptsize (0.30, 0.00) \\
AdVD & & \cellcolor{heatmapgreen!65} 0.128 \scriptsize (0.22, 0.09) & \cellcolor{heatmapgreen!82} 0.063 \scriptsize (0.04, 0.11) & \cellcolor{heatmapgreen!85} 0.054 \scriptsize (0.04, 0.11) & \cellcolor{heatmapgreen!82} 0.062 \scriptsize (0.08, 0.11) &  & \cellcolor{heatmapgreen!88} 0.044 \scriptsize (0.05, 0.00) & \cellcolor{heatmapgreen!82} 0.065 \scriptsize (0.04, 0.17) & \cellcolor{heatmapgreen!74} 0.094 \scriptsize (0.08, 0.14) \\
AdVO & & \cellcolor{heatmapgreen!82} 0.064 \scriptsize (0.04, 0.09) & \cellcolor{heatmapgreen!95} 0.016 \scriptsize (0.02, 0.09) & \cellcolor{heatmapgreen!66} 0.124 \scriptsize (0.09, 0.19) & \cellcolor{heatmapgreen!80} 0.070 \scriptsize (0.10, 0.07) &  & \cellcolor{heatmapgreen!97} 0.008 \scriptsize (0.03, 0.07) & \cellcolor{heatmapgreen!92} 0.027 \scriptsize (0.01, 0.06) & \cellcolor{heatmapgreen!65} 0.125 \scriptsize (0.08, 0.18) \\
DiCO & & \cellcolor{heatmapgreen!0} 0.365 \scriptsize (0.45, 0.35) & \cellcolor{heatmapgreen!67} 0.119 \scriptsize (0.18, 0.00) & \cellcolor{heatmapgreen!64} 0.131 \scriptsize (0.08, 0.45) & \cellcolor{heatmapgreen!66} 0.124 \scriptsize (0.09, 0.22) &  & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) \\
LaMe & & \cellcolor{heatmapgreen!76} 0.087 \scriptsize (0.13, 0.08) & \cellcolor{heatmapgreen!96} 0.013 \scriptsize (0.05, 0.05) & \cellcolor{heatmapgreen!94} 0.021 \scriptsize (0.03, 0.00) & \cellcolor{heatmapgreen!35} 0.236 \scriptsize (0.33, 0.19) &  & \cellcolor{heatmapgreen!92} 0.027 \scriptsize (0.01, 0.04) & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) & \cellcolor{heatmapgreen!80} 0.071 \scriptsize (0.05, 0.09) \\
PaPe & & \cellcolor{heatmapgreen!20} 0.290 \scriptsize (0.45, 0.23) & \cellcolor{heatmapgreen!72} 0.099 \scriptsize (0.17, 0.00) & \cellcolor{heatmapgreen!79} 0.074 \scriptsize (0.07, 0.11) & \cellcolor{heatmapgreen!44} 0.204 \scriptsize (0.45, 0.14) &  & \cellcolor{heatmapgreen!89} 0.039 \scriptsize (0.18, 0.00) & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) & \cellcolor{heatmapgreen!78} 0.080 \scriptsize (0.00, 0.09) \\
PrDE & & \cellcolor{heatmapgreen!48} 0.188 \scriptsize (0.30, 0.14) & \cellcolor{heatmapgreen!84} 0.055 \scriptsize (0.04, 0.09) & \cellcolor{heatmapgreen!95} 0.017 \scriptsize (0.01, 0.00) & \cellcolor{heatmapgreen!53} 0.169 \scriptsize (0.22, 0.14) &  & \cellcolor{heatmapgreen!89} 0.038 \scriptsize (0.02, 0.07) & \cellcolor{heatmapgreen!91} 0.031 \scriptsize (0.02, 0.09) & \cellcolor{heatmapgreen!79} 0.074 \scriptsize (0.10, 0.07) \\
SeVD & & \cellcolor{heatmapgreen!100} 0.000 \scriptsize (0.00, 0.00) & \cellcolor{heatmapgreen!62} 0.138 \scriptsize (0.18, 0.17) & \cellcolor{heatmapgreen!86} 0.051 \scriptsize (0.04, 0.14) & \cellcolor{heatmapgreen!50} 0.183 \scriptsize (0.43, 0.14) &  & \cellcolor{heatmapgreen!92} 0.026 \scriptsize (0.27, 0.00) & \cellcolor{heatmapgreen!75} 0.090 \scriptsize (0.30, 0.00) & \cellcolor{heatmapgreen!73} 0.096 \scriptsize (0.07, 0.09) \\
TrVD & & \cellcolor{heatmapgreen!59} 0.147 \scriptsize (0.45, 0.09) & \cellcolor{heatmapgreen!69} 0.110 \scriptsize (0.12, 0.09) & \cellcolor{heatmapgreen!85} 0.052 \scriptsize (0.04, 0.09) & \cellcolor{heatmapgreen!47} 0.193 \scriptsize (0.24, 0.17) &  & \cellcolor{heatmapgreen!81} 0.066 \scriptsize (0.04, 0.09) & \cellcolor{heatmapgreen!90} 0.036 \scriptsize (0.05, 0.00) & \cellcolor{heatmapgreen!48} 0.187 \scriptsize (0.17, 0.20) \\
\midrule
mean & & \cellcolor{heatmapgreen!61} 0.141 \scriptsize (0.23, 0.12) & \cellcolor{heatmapgreen!79} 0.074 \scriptsize (0.09, 0.10) & \cellcolor{heatmapgreen!83} 0.062 \scriptsize (0.05, 0.12) & \cellcolor{heatmapgreen!56} 0.160 \scriptsize (0.23, 0.18) &  & \cellcolor{heatmapgreen!91} 0.031 \scriptsize (0.07, 0.03) & \cellcolor{heatmapgreen!89} 0.037 \scriptsize (0.05, 0.06) & \cellcolor{heatmapgreen!74} 0.094 \scriptsize (0.10, 0.10) \\


==> tables/large_verification_effort.tex <==
AdCO & 15 & \cellcolor{heatmappurple!0} 0.07 & \cellcolor{heatmappurple!0} 0.50 &  &  & 0 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!100} 0.00 &  & 13 & \cellcolor{heatmapgreen!1} 0.08 & \cellcolor{heatmappurple!0} 0.50 &  & 18 & \cellcolor{heatmapgreen!4} 0.11 & \cellcolor{heatmapgreen!100} 1.00 &  & 5 & \cellcolor{heatmapgreen!14} 0.20 & \cellcolor{heatmappurple!0} 0.50 &  &  & 3 & \cellcolor{heatmapgreen!28} 0.33 & \cellcolor{heatmappurple!0} 0.50 &  & 8 & \cellcolor{heatmapgreen!19} 0.25 & \cellcolor{heatmapgreen!100} 1.00 &  & 3 & \cellcolor{heatmapgreen!28} 0.33 & \cellcolor{heatmappurple!0} 0.50 \\
AdVD & 59 & \cellcolor{heatmappurple!0} 0.07 & \cellcolor{heatmappurple!0} 0.80 &  &  & 2 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!100} 0.00 &  & 19 & \cellcolor{heatmappurple!22} 0.05 & \cellcolor{heatmappurple!75} 0.20 &  & 19 & \cellcolor{heatmapgreen!9} 0.16 & \cellcolor{heatmappurple!25} 0.60 &  & 2 & \cellcolor{heatmapgreen!46} 0.50 & \cellcolor{heatmappurple!75} 0.20 &  &  & 11 & \cellcolor{heatmapgreen!12} 0.18 & \cellcolor{heatmappurple!50} 0.40 &  & 14 & \cellcolor{heatmapgreen!15} 0.21 & \cellcolor{heatmappurple!25} 0.60 &  & 6 & \cellcolor{heatmapgreen!28} 0.33 & \cellcolor{heatmappurple!50} 0.40 \\
AdVO & 10 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!0} 0.50 &  &  & 9 & \cellcolor{heatmappurple!44} 0.22 & \cellcolor{heatmappurple!50} 0.25 &  & 17 & \cellcolor{heatmappurple!41} 0.24 & \cellcolor{heatmappurple!0} 0.50 &  & 16 & \cellcolor{heatmappurple!6} 0.38 & \cellcolor{heatmapgreen!50} 0.75 &  & 3 & \cellcolor{heatmappurple!16} 0.33 & \cellcolor{heatmappurple!75} 0.12 &  &  & 10 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!0} 0.50 &  & 14 & \cellcolor{heatmapgreen!16} 0.50 & \cellcolor{heatmapgreen!75} 0.88 &  & 5 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!50} 0.25 \\
DiCO & 9 & \cellcolor{heatmappurple!0} 0.22 & \cellcolor{heatmappurple!0} 1.00 &  &  & 1 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!50} 0.50 &  & 3 & \cellcolor{heatmapgreen!57} 0.67 & \cellcolor{heatmappurple!0} 1.00 &  & 13 & \cellcolor{heatmappurple!30} 0.15 & \cellcolor{heatmappurple!0} 1.00 &  & 4 & \cellcolor{heatmapgreen!35} 0.50 & \cellcolor{heatmappurple!0} 1.00 &  &  & 3 & \cellcolor{heatmapgreen!57} 0.67 & \cellcolor{heatmappurple!0} 1.00 &  & 4 & \cellcolor{heatmapgreen!35} 0.50 & \cellcolor{heatmappurple!0} 1.00 &  & 3 & \cellcolor{heatmapgreen!57} 0.67 & \cellcolor{heatmappurple!0} 1.00 \\
LaMe & 4 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmappurple!0} 0.20 &  &  & 7 & \cellcolor{heatmapgreen!14} 0.57 & \cellcolor{heatmapgreen!25} 0.40 &  & 10 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmapgreen!37} 0.50 &  & 17 & \cellcolor{heatmapgreen!5} 0.53 & \cellcolor{heatmapgreen!87} 0.90 &  & 6 & \cellcolor{heatmapgreen!33} 0.67 & \cellcolor{heatmapgreen!25} 0.40 &  &  & 12 & \cellcolor{heatmapgreen!16} 0.58 & \cellcolor{heatmapgreen!62} 0.70 &  & 15 & \cellcolor{heatmapgreen!33} 0.67 & \cellcolor{heatmapgreen!100} 1.00 &  & 8 & \cellcolor{heatmapgreen!25} 0.62 & \cellcolor{heatmapgreen!37} 0.50 \\
PaPe & 2 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 &  &  & 2 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 &  & 7 & \cellcolor{heatmappurple!57} 0.43 & \cellcolor{heatmapgreen!33} 0.60 &  & 8 & \cellcolor{heatmappurple!50} 0.50 & \cellcolor{heatmapgreen!66} 0.80 &  & 1 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!50} 0.20 &  &  & 2 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 &  & 5 & \cellcolor{heatmappurple!19} 0.80 & \cellcolor{heatmapgreen!66} 0.80 &  & 2 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 \\
PrDE & 5 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!0} 0.33 &  &  & 3 & \cellcolor{heatmappurple!16} 0.33 & \cellcolor{heatmappurple!49} 0.17 &  & 18 & \cellcolor{heatmappurple!30} 0.28 & \cellcolor{heatmapgreen!74} 0.83 &  & 23 & \cellcolor{heatmappurple!56} 0.17 & \cellcolor{heatmapgreen!49} 0.67 &  & 4 & \cellcolor{heatmappurple!37} 0.25 & \cellcolor{heatmappurple!49} 0.17 &  &  & 12 & \cellcolor{heatmapgreen!2} 0.42 & \cellcolor{heatmapgreen!74} 0.83 &  & 14 & \cellcolor{heatmappurple!10} 0.36 & \cellcolor{heatmapgreen!74} 0.83 &  & 6 & \cellcolor{heatmappurple!16} 0.33 & \cellcolor{heatmappurple!0} 0.33 \\
SeVD & 8 & \cellcolor{heatmappurple!0} 0.25 & \cellcolor{heatmappurple!0} 0.40 &  &  & 0 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!100} 0.00 &  & 5 & \cellcolor{heatmapgreen!20} 0.40 & \cellcolor{heatmappurple!0} 0.40 &  & 10 & \cellcolor{heatmapgreen!6} 0.30 & \cellcolor{heatmapgreen!33} 0.60 &  & 1 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!50} 0.20 &  &  & 1 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!50} 0.20 &  & 2 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!0} 0.40 &  & 2 & \cellcolor{heatmapgreen!33} 0.50 & \cellcolor{heatmappurple!50} 0.20 \\
TrVD & 1 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.17 &  &  & 0 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!99} 0.00 &  & 8 & \cellcolor{heatmappurple!62} 0.38 & \cellcolor{heatmapgreen!40} 0.50 &  & 13 & \cellcolor{heatmappurple!76} 0.23 & \cellcolor{heatmapgreen!40} 0.50 &  & 4 & \cellcolor{heatmappurple!25} 0.75 & \cellcolor{heatmapgreen!40} 0.50 &  &  & 6 & \cellcolor{heatmappurple!33} 0.67 & \cellcolor{heatmapgreen!60} 0.67 &  & 9 & \cellcolor{heatmappurple!55} 0.44 & \cellcolor{heatmapgreen!60} 0.67 &  & 4 & \cellcolor{heatmappurple!25} 0.75 & \cellcolor{heatmapgreen!40} 0.50 \\


==> tables/median_f1_scores.tex <==
AdCO & 0.118 & & \cellcolor{heatmappurple!100} 0.000 & \cellcolor{heatmapgreen!1} 0.133 & \cellcolor{heatmapgreen!9} 0.200 & \cellcolor{heatmapgreen!19} 0.286 & & \cellcolor{heatmapgreen!32} 0.400 & \cellcolor{heatmapgreen!32} 0.400 & \cellcolor{heatmapgreen!32} 0.400 \\
AdVD & 0.125 & & \cellcolor{heatmappurple!100} 0.000 & \cellcolor{heatmappurple!33} 0.083 & \cellcolor{heatmapgreen!14} 0.250 & \cellcolor{heatmapgreen!18} 0.286 & & \cellcolor{heatmapgreen!14} 0.250 & \cellcolor{heatmapgreen!21} 0.316 & \cellcolor{heatmapgreen!27} 0.364 \\
AdVO & 0.444 & & \cellcolor{heatmappurple!47} 0.235 & \cellcolor{heatmappurple!27} 0.320 & \cellcolor{heatmapgreen!10} 0.500 & \cellcolor{heatmappurple!59} 0.182 & & \cellcolor{heatmappurple!0} 0.444 & \cellcolor{heatmapgreen!34} 0.636 & \cellcolor{heatmappurple!30} 0.308 \\
DiCO & 0.364 & & \cellcolor{heatmapgreen!47} 0.667 & \cellcolor{heatmapgreen!68} 0.800 & \cellcolor{heatmappurple!26} 0.267 & \cellcolor{heatmapgreen!47} 0.667 & & \cellcolor{heatmapgreen!68} 0.800 & \cellcolor{heatmapgreen!47} 0.667 & \cellcolor{heatmapgreen!68} 0.800 \\
LaMe & 0.286 & & \cellcolor{heatmapgreen!25} 0.471 & \cellcolor{heatmapgreen!30} 0.500 & \cellcolor{heatmapgreen!53} 0.667 & \cellcolor{heatmapgreen!30} 0.500 & & \cellcolor{heatmapgreen!49} 0.636 & \cellcolor{heatmapgreen!72} 0.800 & \cellcolor{heatmapgreen!37} 0.556 \\
PaPe & 0.571 & & \cellcolor{heatmappurple!0} 0.571 & \cellcolor{heatmappurple!12} 0.500 & \cellcolor{heatmapgreen!10} 0.615 & \cellcolor{heatmappurple!41} 0.333 & & \cellcolor{heatmappurple!0} 0.571 & \cellcolor{heatmapgreen!53} 0.800 & \cellcolor{heatmappurple!0} 0.571 \\
PrDE & 0.364 & & \cellcolor{heatmappurple!38} 0.222 & \cellcolor{heatmapgreen!8} 0.417 & \cellcolor{heatmappurple!24} 0.276 & \cellcolor{heatmappurple!45} 0.200 & & \cellcolor{heatmapgreen!30} 0.556 & \cellcolor{heatmapgreen!21} 0.500 & \cellcolor{heatmappurple!8} 0.333 \\
SeVD & 0.308 & & \cellcolor{heatmappurple!100} 0.000 & \cellcolor{heatmapgreen!13} 0.400 & \cellcolor{heatmapgreen!13} 0.400 & \cellcolor{heatmapgreen!3} 0.333 & & \cellcolor{heatmapgreen!3} 0.333 & \cellcolor{heatmapgreen!38} 0.571 & \cellcolor{heatmappurple!7} 0.286 \\
TrVD & 0.286 & & \cellcolor{heatmappurple!100} 0.000 & \cellcolor{heatmapgreen!19} 0.429 & \cellcolor{heatmapgreen!4} 0.316 & \cellcolor{heatmapgreen!44} 0.600 & & \cellcolor{heatmapgreen!53} 0.667 & \cellcolor{heatmapgreen!34} 0.533 & \cellcolor{heatmapgreen!44} 0.600 \\


==> tables/precision_recall.tex <==
AdCO & \cellcolor{heatmappurple!0} 0.07 & \cellcolor{heatmappurple!0} 0.50 &  & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmapgreen!1} 0.08 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmapgreen!4} 0.11 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmapgreen!14} 0.20 & \cellcolor{heatmappurple!0} 0.50 &  & \cellcolor{heatmapgreen!28} 0.33 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmapgreen!19} 0.25 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmapgreen!28} 0.33 & \cellcolor{heatmappurple!0} 0.50 \\
AdVD & \cellcolor{heatmappurple!0} 0.07 & \cellcolor{heatmappurple!0} 0.80 &  & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!22} 0.05 & \cellcolor{heatmappurple!75} 0.20 & \cellcolor{heatmapgreen!9} 0.16 & \cellcolor{heatmappurple!25} 0.60 & \cellcolor{heatmapgreen!46} 0.50 & \cellcolor{heatmappurple!75} 0.20 &  & \cellcolor{heatmapgreen!12} 0.18 & \cellcolor{heatmappurple!50} 0.40 & \cellcolor{heatmapgreen!15} 0.21 & \cellcolor{heatmappurple!25} 0.60 & \cellcolor{heatmapgreen!28} 0.33 & \cellcolor{heatmappurple!50} 0.40 \\
AdVO & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!0} 0.50 &  & \cellcolor{heatmappurple!44} 0.22 & \cellcolor{heatmappurple!50} 0.25 & \cellcolor{heatmappurple!41} 0.24 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmappurple!6} 0.38 & \cellcolor{heatmapgreen!50} 0.75 & \cellcolor{heatmappurple!16} 0.33 & \cellcolor{heatmappurple!75} 0.12 &  & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmapgreen!16} 0.50 & \cellcolor{heatmapgreen!75} 0.88 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!50} 0.25 \\
DiCO & \cellcolor{heatmappurple!0} 0.22 & \cellcolor{heatmappurple!0} 1.00 &  & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!50} 0.50 & \cellcolor{heatmapgreen!57} 0.67 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!30} 0.15 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmapgreen!35} 0.50 & \cellcolor{heatmappurple!0} 1.00 &  & \cellcolor{heatmapgreen!57} 0.67 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmapgreen!35} 0.50 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmapgreen!57} 0.67 & \cellcolor{heatmappurple!0} 1.00 \\
LaMe & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmappurple!0} 0.20 &  & \cellcolor{heatmapgreen!14} 0.57 & \cellcolor{heatmapgreen!25} 0.40 & \cellcolor{heatmappurple!0} 0.50 & \cellcolor{heatmapgreen!37} 0.50 & \cellcolor{heatmapgreen!5} 0.53 & \cellcolor{heatmapgreen!87} 0.90 & \cellcolor{heatmapgreen!33} 0.67 & \cellcolor{heatmapgreen!25} 0.40 &  & \cellcolor{heatmapgreen!16} 0.58 & \cellcolor{heatmapgreen!62} 0.70 & \cellcolor{heatmapgreen!33} 0.67 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmapgreen!25} 0.62 & \cellcolor{heatmapgreen!37} 0.50 \\
PaPe & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 &  & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!57} 0.43 & \cellcolor{heatmapgreen!33} 0.60 & \cellcolor{heatmappurple!50} 0.50 & \cellcolor{heatmapgreen!66} 0.80 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!50} 0.20 &  & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!19} 0.80 & \cellcolor{heatmapgreen!66} 0.80 & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.40 \\
PrDE & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmappurple!0} 0.33 &  & \cellcolor{heatmappurple!16} 0.33 & \cellcolor{heatmappurple!49} 0.17 & \cellcolor{heatmappurple!30} 0.28 & \cellcolor{heatmapgreen!74} 0.83 & \cellcolor{heatmappurple!56} 0.17 & \cellcolor{heatmapgreen!49} 0.67 & \cellcolor{heatmappurple!37} 0.25 & \cellcolor{heatmappurple!49} 0.17 &  & \cellcolor{heatmapgreen!2} 0.42 & \cellcolor{heatmapgreen!74} 0.83 & \cellcolor{heatmappurple!10} 0.36 & \cellcolor{heatmapgreen!74} 0.83 & \cellcolor{heatmappurple!16} 0.33 & \cellcolor{heatmappurple!0} 0.33 \\
SeVD & \cellcolor{heatmappurple!0} 0.25 & \cellcolor{heatmappurple!0} 0.40 &  & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmapgreen!20} 0.40 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmapgreen!6} 0.30 & \cellcolor{heatmapgreen!33} 0.60 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!50} 0.20 &  & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!50} 0.20 & \cellcolor{heatmapgreen!100} 1.00 & \cellcolor{heatmappurple!0} 0.40 & \cellcolor{heatmapgreen!33} 0.50 & \cellcolor{heatmappurple!50} 0.20 \\
TrVD & \cellcolor{heatmappurple!0} 1.00 & \cellcolor{heatmappurple!0} 0.17 &  & \cellcolor{heatmappurple!100} 0.00 & \cellcolor{heatmappurple!99} 0.00 & \cellcolor{heatmappurple!62} 0.38 & \cellcolor{heatmapgreen!40} 0.50 & \cellcolor{heatmappurple!76} 0.23 & \cellcolor{heatmapgreen!40} 0.50 & \cellcolor{heatmappurple!25} 0.75 & \cellcolor{heatmapgreen!40} 0.50 &  & \cellcolor{heatmappurple!33} 0.67 & \cellcolor{heatmapgreen!60} 0.67 & \cellcolor{heatmappurple!55} 0.44 & \cellcolor{heatmapgreen!60} 0.67 & \cellcolor{heatmappurple!25} 0.75 & \cellcolor{heatmapgreen!40} 0.50 \\


==> tables/verification_effort.tex <==
AdCO & & \cellcolor{heatmapgreen!100} 0 & \cellcolor{heatmapgreen!51} 13 & \cellcolor{heatmapgreen!33} 18 & \cellcolor{heatmapgreen!81} 5 &  & \cellcolor{heatmapgreen!88} 3 & \cellcolor{heatmapgreen!70} 8 & \cellcolor{heatmapgreen!88} 3 \\
AdVD & & \cellcolor{heatmapgreen!92} 2 & \cellcolor{heatmapgreen!29} 19 & \cellcolor{heatmapgreen!29} 19 & \cellcolor{heatmapgreen!92} 2 &  & \cellcolor{heatmapgreen!59} 11 & \cellcolor{heatmapgreen!48} 14 & \cellcolor{heatmapgreen!77} 6 \\
AdVO & & \cellcolor{heatmapgreen!66} 9 & \cellcolor{heatmapgreen!37} 17 & \cellcolor{heatmapgreen!40} 16 & \cellcolor{heatmapgreen!88} 3 &  & \cellcolor{heatmapgreen!62} 10 & \cellcolor{heatmapgreen!48} 14 & \cellcolor{heatmapgreen!81} 5 \\
DiCO & & \cellcolor{heatmapgreen!96} 1 & \cellcolor{heatmapgreen!88} 3 & \cellcolor{heatmapgreen!51} 13 & \cellcolor{heatmapgreen!85} 4 &  & \cellcolor{heatmapgreen!88} 3 & \cellcolor{heatmapgreen!85} 4 & \cellcolor{heatmapgreen!88} 3 \\
LaMe & & \cellcolor{heatmapgreen!74} 7 & \cellcolor{heatmapgreen!62} 10 & \cellcolor{heatmapgreen!37} 17 & \cellcolor{heatmapgreen!77} 6 &  & \cellcolor{heatmapgreen!55} 12 & \cellcolor{heatmapgreen!44} 15 & \cellcolor{heatmapgreen!70} 8 \\
PaPe & & \cellcolor{heatmapgreen!92} 2 & \cellcolor{heatmapgreen!74} 7 & \cellcolor{heatmapgreen!70} 8 & \cellcolor{heatmapgreen!96} 1 &  & \cellcolor{heatmapgreen!92} 2 & \cellcolor{heatmapgreen!81} 5 & \cellcolor{heatmapgreen!92} 2 \\
PrDE & & \cellcolor{heatmapgreen!88} 3 & \cellcolor{heatmapgreen!33} 18 & \cellcolor{heatmapgreen!14} 23 & \cellcolor{heatmapgreen!85} 4 &  & \cellcolor{heatmapgreen!55} 12 & \cellcolor{heatmapgreen!48} 14 & \cellcolor{heatmapgreen!77} 6 \\
SeVD & & \cellcolor{heatmapgreen!100} 0 & \cellcolor{heatmapgreen!81} 5 & \cellcolor{heatmapgreen!62} 10 & \cellcolor{heatmapgreen!96} 1 &  & \cellcolor{heatmapgreen!96} 1 & \cellcolor{heatmapgreen!92} 2 & \cellcolor{heatmapgreen!92} 2 \\
TrVD & & \cellcolor{heatmapgreen!100} 0 & \cellcolor{heatmapgreen!70} 8 & \cellcolor{heatmapgreen!51} 13 & \cellcolor{heatmapgreen!85} 4 &  & \cellcolor{heatmapgreen!77} 6 & \cellcolor{heatmapgreen!66} 9 & \cellcolor{heatmapgreen!85} 4 \\
\midrule
mean & & \cellcolor{heatmapgreen!92} 2 & \cellcolor{heatmapgreen!59} 11 & \cellcolor{heatmapgreen!44} 15 & \cellcolor{heatmapgreen!88} 3 &  & \cellcolor{heatmapgreen!77} 6 & \cellcolor{heatmapgreen!66} 9 & \cellcolor{heatmapgreen!85} 4 \\

